Source-Seeking Problem with Robot Swarms

We present an algorithm to solve the problem of locating the source, or maxima, of a scalar field using a robot swarm. We demonstrate how the robot swarm determines its direction of movement to approach the source using only field intensity measurements taken by each robot. In contrast with the current literature, our algorithm accommodates a generic (non-degenerate) geometry for the swarm's formation. Additionally, we rigorously show the effectiveness of the algorithm even when the dynamics of the robots are complex, such as a unicycle with constant speed. Not requiring a strict geometry for the swarm significantly enhances its resilience. For example, this allows the swarm to change its size and formation in the presence of obstacles or other real-world factors, including the loss or addition of individuals to the swarm on the fly. For clarity, the article begins by presenting the algorithm for robots with free dynamics. In the second part, we demonstrate the algorithm's effectiveness even considering non-holonomic dynamics for the robots, using the vector field guidance paradigm. Finally, we verify and validate our algorithm with various numerical simulations.

==> anexo-english.tex <==
\appendix
\section{Anexo a ``Algoritmo resiliente con garantías formales para la búsqueda de fuentes en campos escalares mediante un enjambre robótico"}\label{appendix-a}


\setcounter{section}{5}
\section{Demostración del Lema III.3.}


\setcounter{section}{3}
\setcounter{theorem}{2}
\begin{lemma}
Sea $\vec{m}_d(t) = \vec{m}_d(\vec{R}(t))$ el campo guía en una trayectoria del enjambre. Entonces
\begin{equation*}
    \dot{\vec{m}}_d(t) = \omega_{d}(\vec{R}(t), \alpha(t)) E \vec{m}_d(t),
\end{equation*}
donde $\omega_{d}: \mathbb{R}^2 \to \mathbb{R}$ es una función continua y únicamente determinada y $E = \Big[\begin{smallmatrix} 0 & -1 \\ 1 & 0\end{smallmatrix}\Big]$.
\end{lemma}
\begin{proof}
Diferenciamos la igualdad $||\vec{m}_d(t)||^2 = 1$ de forma que tenemos $\dot{\vec{m}}_d(t) \cdot \vec{m}_d(t) = 0$, es decir, $\dot{\vec{m}}_d(t) \perp \vec{m}_d(t)$ en cualquier punto de la trayectoria. 

De esta forma, $\dot{\vec{m}}_d(t)$ es proporcional al vector unitario $E m_d(t)$, por lo que $\dot{\vec{m}}_d(t) =  \omega_d(t) E \vec{m}_d(t)$, y el factor escalar $\omega_d(t)$ se puede obtener de
\begin{equation*}
    \omega_d(t) = \dot{\vec{m}}_d(t)^t E \vec{m}_d(t).
\end{equation*}
Falta ver que $\omega_d$ depende solamente de la trayectoria $(\vec{R}(t), \alpha(t))$ y que esta dependencia es continua, pero esto es automático dado que la dependencia de $\vec{m}_d(t)$ es continua en dichos parámetros, al igual que lo es la de $\dot{\vec{m}}_d(t)$.
\end{proof}
\setcounter{section}{6}
\section{Resultados técnicos para la demostración del Teorema III.4.}

Para poder garantizar que la dinámica
\begin{align}
    \dot{\Vec{r}}_i &= u_r \begin{bmatrix} \cos{(\alpha_i)} \\ \sin{(\alpha_i)} \end{bmatrix} \hspace{10 pt} i = 1, \dots, N \nonumber \\
    \dot{\alpha}_i &= \omega_i \hspace{10 pt} i = 1, \dots, N \\
    \dot{\delta}_{i, *} &= \omega_i - \omega_d(\vec{r}), \hspace{10 pt} \delta_{i,*}(0) = \delta_{i}(0), \hspace{10 pt} i = 1, \dots, N \nonumber,
\end{align}
da una solución al problema de búsqueda, hemos de resolver antes ciertos escollos de naturaleza técnica, que recogeremos en esta sección. El primero de estos resultados trata sobre la estabilidad de la geometría del enjambre, garantizándonos que, bajo ciertas condiciones, podemos controlar cuánto se deformará.

\begin{lemma}\label{lema-estabilidad}
    Supongamos que $\vec{R}(t)$ es una trayectoria del sistema de ecuaciones diferenciales \eqref{eq:augmentado}, entonces se sigue que
    \begin{equation*}
        \norm{\vec{r}_{i,j}(t) - \vec{r}_{i,j}(0)} \leq 2\pi \frac{u_r}{k_\gamma}, \hspace{10 pt} \forall \hspace{3 pt} 1 \leq i < j \leq N
    \end{equation*}   
    donde $\vec{r}_{i,j} = \vec{r}_i - \vec{r}_j$.
\end{lemma}

\begin{proof}
Definimos
\begin{equation*}
    \delta_{i,j} = \alpha_j - \alpha_i,
\end{equation*}
que corresponde con el ángulo orientado partiendo de la velocidad del robot $i$ hacia la del robot $j$. Notamos que\footnote{Esto se debe a cómo estamos midiendo los ángulos, puede que los midamos por el camino más largo.} $\delta_{i,j} \in (-2\pi, 2\pi)$, de forma que $\delta_{i,j} = 0$ nos indica que ambos robots apuntan en la misma dirección. Además, es fácil comprobar que
\begin{equation*}
    \delta_{i,j} = \delta_{j,*} - \delta_{i,*}.
\end{equation*}
De esta forma, tenemos que
\begin{equation*}
    \dot{\delta}_{i,j} = \omega_j - \omega_i = -k_\gamma (\delta_{j,*} - \delta_{i,*}) = - k_\gamma \delta_{i,j},
\end{equation*}
o lo que es lo mismo, en la trayectoria del sistema
\begin{equation*}
    \delta_{i,j} = \delta_{i,j}(0) e^{-k_\gamma t},
\end{equation*}
por lo que $\delta_{i,j} \to 0$ cuando $t \to \infty$. Con esto, estamos listos para evaluar la deformación del sistema, ya que se tiene fácilmente que
\begin{align*}
    \dot{\Vec{r}}_{i,j} &= \dot{\Vec{r}}_{i} - \dot{\Vec{r}}_{j} = u_r \begin{bmatrix} \cos(\alpha_i) - \cos{(\alpha_j)}  \\ \sin(\alpha_i) - \sin(\alpha_j) \end{bmatrix} = 2u_r \sin\left( \frac{\alpha_j - \alpha_i}{2}\right) \begin{bmatrix} \sin\left( \frac{\alpha_i + \alpha_j}{2}\right) \\ - \cos\left( \frac{\alpha_i + \alpha_j}{2}\right)\end{bmatrix} \\
    &= 2u_r \sin\left( \frac{\delta_{i,j}}{2}\right) \begin{bmatrix} \sin\left( \frac{\alpha_i + \alpha_j}{2}\right) \\ - \cos\left( \frac{\alpha_i + \alpha_j}{2}\right)\end{bmatrix} = 2u_r \sin\left(\frac{\delta_{i,j}(0)e^{-k_\gamma t}}{2} \right) \begin{bmatrix} \sin\left( \frac{\alpha_i + \alpha_j}{2}\right) \\ - \cos\left( \frac{\alpha_i + \alpha_j}{2}\right)\end{bmatrix}.
\end{align*}
De esta forma se sigue que
\begin{equation*}
    ||\dot{\Vec{r}}_{i,j}|| \leq 2u_r \left | \sin\left(\frac{\delta_{i,j}(0)e^{-k_\gamma t}}{2}  \right) \right| \leq u_r |\delta_{i,j}(0)| e^{-k_\gamma t},
\end{equation*}
por lo que rápidamente se estabiliza la posición. En efecto, tenemos que podemos escribir
\begin{equation*}
    \Vec{r}_{i,j}(t) = \Vec{r}_{i,j}(0) + \int_0^t \dot{\Vec{r}}_{i,j},
\end{equation*}
y por tanto
\begin{align*}
    \norm{\Vec{r}_{i,j}(t) - \Vec{r}_{i,j}(0)} &= \norm{ \int_0^t \dot{\Vec{r}}_{i,j}} \leq \int_0^t ||\dot{\Vec{r}}_{i,j}|| \leq u_r |\delta_{i,j}(0)| \int_0^t e^{-k_\gamma t} \\
    &\leq u_r |\delta_{i,j}(0)| \int_0^\infty e^{-k_\gamma t} = \frac{u_r |\delta_{i,j}(0)|}{k_\gamma} \leq 2\pi \frac{u_r}{k_\gamma},
\end{align*}
donde hemos usado que $\delta_{i,j}(0) \in (-2\pi, 2\pi)$.
\end{proof}
\begin{corollary}\label{corolario-estabilidad}
    Si $\vec{R}(t)$ es una trayectoria del sistema de ecuaciones diferenciales de \eqref{eq:augmentado}, entonces se tiene
        \begin{equation*}
            \norm{\vec{x}_{i}(t) - \vec{x}_{i}(0)} \leq 2\pi \frac{u_r}{k_\gamma}.
        \end{equation*}
\end{corollary}
El resultado anterior nos garantiza que, siempre que la velocidad angular sea lo suficientemente rápida con respecto a la velocidad linear, lograremos que la geometría del sistema se estabilice rápidamente cuando siga al campo.

El segundo resultado de esta sección trata con la necesidad de acotar superiormente $|\omega_d|$ en nuestra trayectoria. Esto último no es del todo posible. La razón es la siguiente: si $\vec{r}^*$ representa un máximo de la señal, entonces $\grad \sigma(\vec{r}^*) = 0$, de forma que $\vec{m}_d$ no está bien definida en ese punto\footnote{Técnicamente, en todo el subconjunto de $\mathbb{R}^{2N}$ tal que $\vec{r}_c = \vec{r}^*$.}. Más importante, en un entorno lo suficientemente pequeño de $\vec{r}^*$, la velocidad angular $\omega_d$ cambia rápidamente, pues al pasar por el punto $\vec{r}^*$ el vector $\omega_d$ da un giro \emph{instantáneo} de $180$ grados. Para lidiar con estas dificultades técnicas, nos restringiremos a trayectorias que se encuentren alejadas de esta clase de entornos, de forma que en última instancia podemos garantizar que nuestro sistema de robots se acerca a dichos entornos\footnote{Lo cuál es suficiente, pues estamos localizando un entorno que contiene el máximo de nuestra señal.}, aunque no su comportamiento en los mismos.

Antes de poder probar este resultado, nos hará falta un resultado previo.

\begin{lemma}\label{lema-lower_bound}
     Sea $\vec{R}(t)$ una de trayectoria del sistema de ecuaciones \eqref{eq:augmentado} con geometría inicial $\vec{X}(0)$ no degenerada. Entonces existen constantes $\kappa, m > 0$ de forma que si $k_\gamma \geq \kappa$ entonces $\norm{\vec{L}_\sigma(\vec{R}(t))} \geq m || \grad \sigma(\vec{r}_c(t)) ||$.
\end{lemma}
\begin{proof}
    Dado que $\vec{X}(0)$ es no degenerada, podemos asumir sin pérdida de generalidad que $\vec{x}_1(0)$ y $\vec{x}_2(0)$ forman base y, por tanto, una ligera perturbación de los mismos seguirá formando base. De esta manera, usando el Corolario \ref{corolario-estabilidad}, existe $\kappa_1 > 0$ tal que si $k_\gamma \geq \kappa_1$ se tiene que $\vec{x}_1(t)$, $\vec{x}_2(t)$ son siempre base.
    
    Por un lado tenemos que
    \begin{equation*}
        \vec{L}_\sigma(\vec{R}) \cdot \grad \sigma(\vec{r}_c) \leq \norm{\vec{L}_\sigma(\vec{R})} \norm{\grad \sigma(\vec{r}_c)},
    \end{equation*}
    mientras que por el Lema III.3 en el documento principal y dado que $\vec{X}$ es no degenerada durante la trayectoria, existen constantes $C(\vec{X})$ tales que
    \begin{equation*}
        \vec{L}_\sigma(\vec{R}) \cdot \grad \sigma(\vec{r}_c) \geq \frac{1}{C(\vec{X})} || \grad \sigma (\vec{r}_c)||^2.
    \end{equation*}
    Es fácil ver, además, que $C(\vec{X})$ se puede escoger como una función continua de la geometría $\vec{X}$. Sabemos, de nuevo por el Corolario \ref{corolario-estabilidad}, que tomando $\kappa_2$ lo suficientemente grande, entonces si $k_\gamma \geq \kappa_2$ se sigue que $\vec{X}(t)$ está contenido en un compacto $F \subset \mathbb{R}^{2N}$ y por tanto $C(\vec{X})$ alcanza su valor máximo en dicho compacto $F$, para cierta geometría $\vec{X}^*$. De esta forma, tomando $C^* = C(\vec{X}^*)$ se tiene que, durante toda la trayectoria,
    \begin{equation*}
        \vec{L}_\sigma(\vec{R}) \cdot \grad \sigma(\vec{r}_c) \geq \frac{1}{C(\vec{X})}   || \grad \sigma (\vec{r}_c)||^2 \geq \frac{1}{C^* }   || \grad \sigma (\vec{r}_c)||^2.
    \end{equation*}
    Combinando esto con lo anterior se tiene
    \begin{equation*}
        \frac{1}{C^* }   || \grad \sigma (\vec{r}_c)||^2 \leq \vec{L}_\sigma(\vec{R}) \cdot \grad \sigma(\vec{r}_c) \leq \norm{\vec{L}_\sigma(\vec{R})} \norm{\grad \sigma(\vec{r}_c)},
    \end{equation*}
    y por tanto
    \begin{equation*}
        \frac{1}{C^* }   || \grad \sigma (\vec{r}_c)|| \leq \norm{\vec{L}_\sigma(\vec{R})}.
    \end{equation*}
    Tomando $m  = 1/C^*$ y $\kappa = \max{\{\kappa_1, \kappa_2\}}$ se sigue el resultado.
\end{proof}

Con esto, ya estamos preparados para probar la cota de la velocidad angular.

\begin{lemma}\label{lema-cotaomega}
    Sea $\vec{R}(t)$ una trayectoria del sistema de ecuaciones \eqref{eq:augmentado} con geometría inicial $\vec{X}(0)$ no degenerada y $\epsilon > 0$ fijado. Entonces existe una constante $\kappa > 0$ tal que si $k_\gamma \geq \kappa$ y $||\grad \sigma (\vec{r}_c(t))|| \geq \epsilon$ entonces $|\omega_d| \leq  \Omega_d$ para cierta constante $\Omega_d(\epsilon)$.
\end{lemma}
\begin{proof}
Recordamos que
\begin{equation*}
    \omega_d(t) =  \dot{\Vec{m}}_d(t)^T E \Vec{m}_d(t),
\end{equation*}
de forma que
\begin{equation*}
    |\omega_d(t)| \leq ||\dot{\Vec{m}}_d(t)|| \norm{\Vec{m}_d(t)} = ||\dot{\Vec{m}}_d(t)||,
\end{equation*}
por lo que una cota de $||\dot{\Vec{m}}_d(t)||$ nos dará una cota a $\omega_d$. 

Además, sabemos que
\begin{equation}\label{eq:CGI-grad}
    \vec{m}_d = \frac{\vec{L}_\sigma(\Vec{R})}{\norm{\vec{L}_\sigma(\Vec{R})}} = \frac{\sum_{i=1}^N (\vec{\nabla} \sigma (\vec{r}_c)  \cdot (\vec{r}_i - \vec{r}_c)) (\vec{r}_i - \vec{r}_c))}{\norm{\sum_{i=1}^N (\vec{\nabla} \sigma (\vec{r}_c)  \cdot (\vec{r}_i - \vec{r}_c)) (\vec{r}_i - \vec{r}_c)) }}.
\end{equation}
Derivando uno de los términos en la suma se tiene que
\begin{align*}
    \frac{d}{dt}\left( \vec{\nabla} \sigma (\vec{r}_c)  \cdot (\vec{r}_i - \vec{r}_c) (\vec{r}_i - \vec{r}_c)\right) &= \left(H_\sigma (\vec{r}_c) \cdot(\vec{r}_i - \vec{r}_c) + \vec{\nabla} \sigma (\vec{r}_c)  \cdot (\dot{\vec{r}}_i - \dot{\vec{r}}_c) \right)(\vec{r}_i - \vec{r}_c) \\
    &+ \vec{\nabla} \sigma (\vec{r}_c)  \cdot (\vec{r}_i - \vec{r}_c) (\dot{\vec{r}}_i - \dot{\vec{r}}_c).
\end{align*}

Por el Corolario \ref{corolario-estabilidad}, en la trayectoria tenemos $\norm{\vec{r}_i - \vec{r}_c} = \norm{\vec{x}_i} \leq \frac{2\pi u_r}{k_\gamma} + \norm{\vec{x}_i(0)} \leq M_1$, donde tomamos $k_\gamma \geq 1$. Ahora, también tenemos que
\begin{equation*}
    ||\dot{\vec{r}}_i - \dot{\vec{r}}_c|| = \norm{\dot{\vec{r}}_i - \frac{1}{N} \sum_{j=1}^N \dot{\vec{r}}_k} \leq u_r + u_r = 2u_r,
\end{equation*}
por lo que también está fácilmente acotado. Finalmente, los términos del Hessiano y el gradiente están acotados por
\begin{equation}
    || \vec{\nabla} \sigma (\vec{r}) || \leq K \hspace{10 pt} \text{ y } \hspace{10 pt} || H_\sigma(\vec{r}) || \leq 2M \hspace{10 pt}, \forall \vec{r} \in \mathbb{R}^2.\nonumber
\end{equation}

De este modo se sigue que
\begin{equation*}
    \norm{\frac{d \vec{L}_\sigma(\vec{R})}{dt}} \leq N\left[2M M_1^2  + 4u_r K M_1 \right] \leq C_1^* 
\end{equation*}
para cierta constante global $C_1^*$. 
Por otro lado se tiene que
\begin{equation*}
    \frac{d}{dt}\norm{\vec{L}_\sigma(\vec{R})} = \frac{1}{2\norm{\vec{L}_\sigma(\vec{R})}}\frac{d}{dt}\norm{\vec{L}_\sigma(\vec{R})}^2 = \frac{\dot{\vec{L}}_\sigma(\vec{r}) \cdot \vec{L}_\sigma(\vec{R})}{\norm{\vec{L}_\sigma(\vec{R})}},
\end{equation*}
por tanto
\begin{equation*}
    \frac{d}{dt}\norm{\vec{L}_\sigma(\vec{R})} \leq \norm{\frac{d \vec{L}_\sigma(\vec{R})}{dt}} \leq C_1^* .
\end{equation*}
Combinando lo anterior tenemos que
\begin{align}
    \norm{\frac{d}{dt} \vec{m}_d} &\leq \frac{2C_1^*  \norm{\vec{L}_\sigma(\vec{R})}}{\norm{\vec{L}_\sigma(\vec{R})}^2} = \frac{2C_1^* }{\norm{\vec{L}_\sigma(\vec{R})}} \leq \frac{2C_1^* }{m  \epsilon} = \Omega_d.
\end{align}
donde la última desigualdad se da tomando $k_\gamma \geq \kappa_1$ dado por el Lema \ref{lema-lower_bound}, junto a la asunción $|| \grad \sigma (\vec{r}_c(t))|| \geq \epsilon$. Tomando $\kappa = \max{\{\kappa_1, 1\}}$ se sigue el resultado.
\end{proof}

Este lema será de gran utilidad en conjunción con el siguiente resultado, que nos dará finalmente una forma de controlar la diferencia de ángulos $\delta_{i,*}$ durante la trayectoria.

\begin{lemma}\label{lema-gamma}
    Para todo ángulo $0 < \gamma < \pi/2$ y para todo $\epsilon > 0$ existe una constante $\kappa > 0$ y un tiempo $t^*$ tal que si $k_\gamma \geq \kappa$ y $|| \grad \sigma(\vec{r}_c(0))|| > \epsilon$ entonces $|\delta_{i,*}(t^*)| < \gamma$, $\forall i = 1, \dots, N$. Además, para $t_0 \geq t^*$ esta cota sigue siendo válida mientras $|| \grad \sigma(\vec{r}_c(t))|| > \epsilon$, $\forall t \in [t^*, t_0)$.
\end{lemma}
\begin{proof}
Sea $\gamma$ y  $\epsilon > 0$ fijados. Como $|| \grad \sigma(\vec{r}_c(0))|| > \epsilon$, se tiene que denotando
$E = \left\{\vec{y}\in \mathbb{R}^2: \norm{\grad \sigma(\vec{y})} \leq \epsilon \right \}$ entonces $dist{(\vec{r}_c(0), E)} = d> 0$. En particular, y dado que $||\dot{\vec{r}}_c|| \leq u_r$, para $t^* = \frac{d}{2u_r}$ se tiene que $\forall t \in [0, 2t^*)$ entonces $|| \grad \sigma(\vec{r}_c(t))|| > \epsilon$.

Por tanto, en el intervalo $[0, t^*]$ estamos en las condiciones del Lema \ref{lema-cotaomega}. Es decir, existe $\kappa_1$ tal que para $k_\gamma \geq \kappa_1$, tenemos que $|\omega_d| \leq \Omega_d$. En particular para todo $k_\gamma \geq \kappa = \max{\left\{\kappa_1, \frac{2\Omega_d}{\gamma}, \frac{2}{t^*}\ln{\left(\frac{\pi}{\gamma} \right)}\right \}}$ se sigue que si $\delta_{i,*} \geq \gamma$ entonces
\begin{equation*}
    \dot{\delta}_{i,*} \leq -k_{\gamma} \delta_{i,*} + \Omega_d \leq -k_\gamma \delta_{i,*} + k_\gamma \frac{\delta_{i,*}}{2} =  -k_\gamma \frac{\delta_{i,*}(t)}{2},
\end{equation*}
mientras que si $\delta_{i,*} \leq - \gamma$ tenemos
\begin{equation*}
    \dot{\delta}_{i,*} \geq - k_\gamma \delta_{i,*} - \Omega_d \geq - k_\gamma \frac{\delta_{i,*}}{2}.
\end{equation*}
Esto implica que $(-\gamma, \gamma)$ es un intervalo atractor. Más particularmente, dada la unicidad de soluciones, una vez dentro de este intervalo y si se sigue cumpliendo la cota para el gradiente, no es posible salir del mismo. 

Por lo tanto, solo hemos de demostrar que caemos dentro de este intervalo para algún $t < t^*$. Si $|\delta_{i,*}(0)| \leq \gamma$, ya hemos explicado que nos quedamos en el intervalo. En otro caso, asumiremos que $\delta_{i,*}(0) \geq \gamma$ y el caso $\delta_{i,*}(0) \leq -\gamma$ se realiza de forma análoga. 
Tenemos que, mientras que $\delta_{i,*}(t)$ no esté dentro del intervalo $(-\gamma, \gamma)$, entonces
\begin{equation*}
    \dot{\delta}_{i,*} \leq -k_\gamma \delta_{i,*}/2 \implies \delta_{i,*}(t) \leq \delta_{i,*}(0)e^{-k_\gamma t/2},
\end{equation*}
y dado que para $t=t^*$ el lado derecho de la desigualdad es estrictamente menor que $\gamma$, en algún momento se tiene que haber entrado dentro del intervalo y, como el intervalo es atractor, seguiremos dentro de él en tiempo $t^*$, como queríamos ver. El hecho de que la cota para $\delta_{i,*}$ se siga cumpliendo mientras $|| \grad \sigma(\vec{r}_c(t))|| > \epsilon$ es automático.
\end{proof}


Por último, destacar que estas dificultades técnicas no tienen demasiada relevancia en la aplicación real, y son resultados meramente necesarios para el tratamiento formal matemático. En efecto, detalles como que la geometría $\vec{X}$ sea no degenerada, si bien necesario para el desarrollo teórico, es prácticamente despreciable en la aplicación real. Similarmente ocurre con las cotas de $\omega_d$, que pueden tomarse como supuestos de buen comportamiento sobre el campo $\vec{m}_d$ si se considerase oportuno. En resumen, los lemas técnicos sirven para justificar la idea natural de que la velocidad angular de los robots es lo suficientemente rápida para seguir adecuadamente el cambio en el campo y que, una vez los robots se alineen con el campo, su geometría se mantendrá casi rígida.

\subsection{Demostración del Teorema III.4.}
Valiéndonos de los resultados anteriormente probados, estamos listos para dar una prueba de convergencia del sistema en \eqref{eq:augmentado}, al menos a entornos donde el gradiente es pequeño, donde esto último viene controlado por el valor de $\epsilon$ que elijamos.

\setcounter{theorem}{3}
\setcounter{section}{3}
\begin{theorem}
    Sea $\sigma$ una distribución de señal, $\vec{R}_0^T = (\vec{r}_{1,0}^T, \dots, \vec{r}_{N,0}^T)^T$ con geometría no degenerada, direcciones de velocidad $\alpha_0 = (\alpha_{1,0}, \dots, \alpha_{N,0})$ y $\epsilon > 0$ fijado. Entonces existe $k_\gamma$ de forma que la dinámica
    \begin{align*}
    \dot{\Vec{r}}_i &= u_r \begin{bmatrix} \cos{(\alpha_i)} \\ \sin{(\alpha_i)} \end{bmatrix}, \hspace{10 pt} \vec{r}_i(0) = \vec{r}_{i,0} \hspace{10 pt} i = 1, \dots, N \nonumber \\
    \dot{\alpha}_i &= -k_\gamma \delta_{i,*}, \hspace{10 pt} \alpha_i(0) = \alpha_{i,0} \hspace{10 pt} i = 1, \dots, N \\
    \dot{\delta}_{i, *} &= -k_\gamma \delta_{i,*} - \omega_d(\vec{r}), \hspace{10 pt} \delta_{i,*}(0) = \delta_{i}(0), \hspace{10 pt} i = 1, \dots, N \nonumber,
    \end{align*}
    es una solución del problema de búsqueda.
\end{theorem}
\begin{proof}
Veremos que existe $k_\gamma$ de forma que el centroide de las trayectorias queda atrapado en el conjunto abierto
\begin{equation*}
    B = \left\{\vec{y} \in \mathbb{R}^2: \norm{\vec{r}^* - \vec{y}} < \epsilon \right\}.
\end{equation*} 
Como hicimos anteriormente, asumiremos sin pérdida de generalidad que $\vec{x}_1(0)$ y $\vec{x}_2(0)$ forman base y razonando como en el Lema \ref{lema-lower_bound} podemos tomar $\kappa_1$ lo suficientemente grande para que $\vec{x_1}(t)$ y $\vec{x}_2(t)$ sean siempre base del espacio y $\vec{X}$ caiga dentro de un compacto.

Queremos estudiar en primer lugar el ángulo que forma nuestro campo guía $\vec{m}_d$ con $\grad \sigma (\vec{r}_c)$, para lo que nos vale estudiar el ángulo entre $\frac{\vec{L}_\sigma(\vec{R})}{{\norm{\grad \sigma (\vec{r}_c)}}}$ y $\frac{\grad \sigma (\vec{r}_c)}{\norm{\grad \sigma (\vec{r}_c)}}$, que denotaremos por $\theta(t)$. Tomando el producto escalar se tiene
\begin{equation*}
     H\left(\vec{X}, \frac{\grad \sigma (\vec{r}_c)}{\norm{\grad \sigma (\vec{r}_c)}}\right) := \frac{\vec{L}_\sigma({\vec{R}(t)}) \cdot \grad \sigma(\vec{r}_c)}{\norm{\grad \sigma(\vec{r}_c(t))}^2} =
         \frac{1}{ND^2}\sum_{i=1}^N \left| \frac{\grad \sigma(\vec{r}_c)}{\norm{\grad \sigma(\vec{r}_c)}} \cdot \vec{x}_i \right|^2 > 0,
\end{equation*}
de forma que $H$ es una función continua en sus parámetros. El primer parámetro $\vec{X}$ está contenido en un compacto $F$, mientras que el segundo parámetro se mueve a lo largo de la esfera unidad $\mathbb{S}$, de forma que la función $H$ en el compacto $F \times \mathbb{S}$ alcanza su mínimo valor $H^* > 0$.  De este modo tenemos que
\begin{equation*}
    0 < H^* \leq \frac{\vec{L}_\sigma({\vec{R}}) \cdot \grad \sigma(\vec{r}_c)}{\norm{\grad \sigma(\vec{r}_c)}^2} = \cos{(\theta)} \frac{\norm{\vec{L}_\sigma({\vec{R}})}}{\norm{\grad \sigma(\vec{r}_c)}} \leq  \cos{(\theta)},
\end{equation*}
donde en la última desigualdad se ha utilizado el hecho de que
\begin{align*}
    \norm{\vec{L}_\sigma({\vec{R}})} &= \frac{1}{ND^2} \norm{\sum_{i=1}^N (\grad \sigma(\vec{r}_c) \cdot \vec{x}_i) \vec{x}_i} \leq \frac{||\grad \sigma(\vec{r}_c)|| }{N} \sum_{i=1}^N \frac{\norm{\vec{x}_i}^2}{D^2} \leq ||\grad \sigma(\vec{r}_c)|| .
\end{align*}
Con esto, se tiene rápidamente que
\begin{equation*}
    0 < H^* \leq  \cos{(\theta)}.
\end{equation*}
De esta forma, sabemos que $|\theta| \leq \arccos{\left(H^*\right)} < \frac{\pi}{2}$. En particular, existe $\gamma > 0$ de forma que $|\theta(t) + \gamma| < \frac{\pi}{2}$ a lo largo de la trayectoria. 

Sea $\epsilon^*$ lo suficientemente pequeño para que 
\begin{equation*}
    A = \left\{\vec{y} \in B: \norm{\grad \sigma(y)} \leq \epsilon^* \right\} \subset  B
\end{equation*}
cumpla que
\begin{equation*}
    d = dist{\left(A, \mathbb{R}^2\backslash B \right)} > 0.
\end{equation*}
Aplicando el Lema \ref{lema-gamma} para dicho $\epsilon^*$ y $\gamma$, se tiene que existe $\kappa_2$ tal que si $k_\gamma \geq \kappa_2$ entonces existe $t^*$ tal que $|\delta_{i,*}(t)| < \gamma, \forall i = 1, \dots, N$ a partir de dicho tiempo $t^*$ y hasta que $\norm{\grad \sigma(\vec{r}_c(t))} \leq \epsilon^*$. En particular, mientras se den las condiciones, la función $\sigma(\vec{r}_c(t))$ es creciente ya que
\begin{equation*}
    \frac{d}{dt}\sigma(\vec{r}_c(t)) = \frac{d \vec{r}_c(t)}{dt} \cdot \grad \sigma(\vec{r}_c(t)) = \frac{u_r}{N} \sum_{i=1}^N \vec{m}_i(\alpha_i(t)) \cdot \grad \sigma(\vec{r}_c(t)) > 0,
\end{equation*}
donde hemos usado que $\vec{m}_i(t) \cdot \grad \sigma(\vec{r}_c(t)) > 0$ por la relación angular previamente probada. Razonando como en el Teorema III.1 en el documento principal, la trayectoria irá al máximo hasta que entre en el conjunto $A$. Una vez dentro, ya no podemos controlar $\sigma(\vec{r}_c(t))$, pero seguimos sabiendo que $\vec{X}$ es estable. De esta forma, si la trayectoria escapa de $A$, tenemos que razonando como en el Lema \ref{lema-gamma} si tomamos $k_\gamma \geq \kappa_3 = \max{\left\{\kappa_4, \frac{2\Omega_d}{\gamma}, \frac{2u_r}{d}\ln{\left(\frac{\pi}{\gamma} \right)}\right\}}$ donde $\kappa_4$ viene dado por el Lema \ref{lema-cotaomega} con $\norm{\grad (\sigma(\vec{r}_c(t))} \geq \epsilon^*$, entonces $|\delta_{i,*}(t)| < \gamma$, $\forall  i = 1, \dots, N$ antes de poder llegar a escapar de $B$, de forma que volverá a acercarse al máximo hasta caer en $A$, y así reiteradamente. Por tanto, para $k_\gamma \geq \kappa = \max{\{\kappa_1, \kappa_2, \kappa_3\}}$ se sigue que la trayectoria queda atrapada en el conjunto $B$, en particular, existe un tiempo $t_0$ tal que para todo $t \geq t_0$ entonces $\norm{\vec{r}^* - \vec{r}_c(t)} < \epsilon$, como queríamos ver.
\end{proof}

Nótese como, en contraposición con el Teorema III.1 en el documento principal donde la dinámica era válida para cualquier $\epsilon$, en este caso, la dinámica es dependiente del $\epsilon$ elegido en el problema de búsqueda. Esto es natural, dado que los robots nunca paran de moverse, siempre rotarán en torno al máximo y el cociente $u_r/k_\gamma$ nos dirá cuán grande será la región sobre la que discurra el enjambre.
